Enabling Faster Locomotion of Planetary Rovers with a Mechanically-Hybrid Suspension

The exploration of the lunar poles and the collection of samples from the martian surface are characterized by shorter time windows demanding increased autonomy and speeds. Autonomous mobile robots must intrinsically cope with a wider range of disturbances. Faster off-road navigation has been explored for terrestrial applications but the combined effects of increased speeds and reduced gravity fields are yet to be fully studied. In this paper, we design and demonstrate a novel fully passive suspension design for wheeled planetary robots, which couples for the first time a high-range passive rocker with elastic in-wheel coil-over shock absorbers. The design was initially conceived and verified in a reduced-gravity (1.625 m/s${^2}$) simulated environment, where three different passive suspension configurations were evaluated against steep slopes and unexpected obstacles, and later prototyped and validated in a series of field tests. The proposed mechanically-hybrid suspension proves to mitigate more effectively the negative effects (high-frequency/high-amplitude vibrations and impact loads) of faster locomotion (~1\,m/s) over unstructured terrains under varied gravity fields.

==> macrosForEThesis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   macrosForEThesis.tex
%%   -------------------
%%
%%   Title: LaTeX macro file for the English Thesis
%%   
%%   
%%   Belief:
%%   1."Fig. 1: ~~~", "Table 1: ~~~" are for the figure and table citation.
%%   2. add the config to read the source code file (hello.c) and visualize it. 
%%
%%   Change Log:
%%   2020.11.26 Initial creation by Kentaro UNO
%%
%%   Contact:
%%   Please contact the author Kentaro UNO (unoken.astro@gmail.com) if
%%   you have a problem
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% useful command
\newcommand{\n}{\nonumber \\}
\newcommand{\p}{\partial}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\II}{I\negthinspace I}
\newcommand{\III}{I\negthinspace I\negthinspace I}
\newcommand{\mbm}[1]{\mbox{\protect \boldmath $#1$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  config for citation of figures, tables, and equations
%%%  to use English for all. 
%%%  2020.01.29 modified by Kentaro UNO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% figure and table
\captionsetup{compatibility=false}
%
\renewcommand{\figurename}{Fig.~\hspace{-.2em}}   
\renewcommand{\tablename}{Table~\hspace{-.2em}}

\captionsetup[figure]{format=plain,labelformat=simple,labelsep=colon,font=small}
\captionsetup[table]{format=plain,labelformat=simple,labelsep=colon,font=small}

\newcommand{\bhline}[1]{\noalign{\hrule height #1}} % bhlineコマンドの設定

%%% citation command for figures, tables, and equations
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\subfig}[2]{Fig.~\ref{#1}\subref{#2}}
\newcommand{\fign}[1]{\ref{#1}}
\newcommand{\tb}[1]{Table~\ref{#1}}
\newcommand{\tabn}[1]{\ref{#1}}
\newcommand{\eq}[1]{Eq.~(\ref{#1})}
\newcommand{\eqn}[1]{(\ref{#1})}

%%% citation command for chapters, sections, and appendixes
\newcommand{\chap}[1]{Chap.~\ref{#1}}
\newcommand{\sect}[1]{Sect.~\ref{#1}}
\newcommand{\subsect}[1]{Sect.~\ref{#1}}
\newcommand{\app}[1]{Appnd. ~\ref{#1}}

%%% visualize a figure and table in a row
\makeatletter
\newcommand{\figcaption}[1]{\def\@captype{figure}\caption{#1}}
\newcommand{\tblcaption}[1]{\def\@captype{table}\caption{#1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  ソースコードの引用スタイルの設定
%%%  2020.01.24 added by Kentaro UNO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings} %日本語のコメントアウトをする場合はjlistingが必要
%ここからソースコードの表示に関する設定
\definecolor{gray}{rgb}{0.9,0.9,0.9}
\lstset{
  backgroundcolor=\color{gray}, % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle={\small\ttfamily}, % the style of the fonts that are used for the code
  identifierstyle={\small}, % main()の''main''等のスタイル
  commentstyle={\small\itshape}, %//comment 等のスタイル
  keywordstyle={\small}, % int mainの''int''等のスタイル
  ndkeywordstyle={\small},
  stringstyle={\small\ttfamily},  % string literal style -> % printf(''Hello'')の''''で囲まれた部分のスタイル
  %frame={tb},
  breaklines=true, % sets automatic line breaking
  columns=[l]{fullflexible},
  numbers=left, % where to put the line-numbers; possible values are (none, left, right)
  numberstyle={\scriptsize}, % the style that is used for the line-numbers
  stepnumber=1, % the step between two line-numbers. If it's 1, each line will be numbered
  numbersep=1zw, % 行数字とコードの間のマージン
  xrightmargin=0zw, % 表示個所の右側マージン
  xleftmargin=2zw,  % 表示個所の左側マージン
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  lineskip=-0.5ex % codeの行間の設定
}

\def\epsgaiji#1{\leavevmode\kern-0.025zw\raise-.37zh\hbox{%
  \epsfile{file=#1,width=1.05zw}}\kern-0.025zw}
%\newcommand{\dfrac}[2]{\frac{\displaystyle{#1}}{\displaystyle{#2}}}
\newcommand{\MARU}[1]{{\ooalign{\hfil#1\/\hfil\crcr\raise.167ex\hbox{\mathhexbox20D}}}}

%%%
